Designing ReachBot: System Design Process with a Case Study of a Martian Lava Tube Mission

In this paper we present a trade study-based method to optimize the architecture of ReachBot, a new robotic concept that uses deployable booms as prismatic joints for mobility in environments with adverse gravity conditions and challenging terrain. Specifically, we introduce a design process wherein we analyze the compatibility of ReachBot's design with its mission. We incorporate terrain parameters and mission requirements to produce a final design optimized for mission-specific objectives. ReachBot's design parameters include (1) number of booms, (2) positions and orientations of the booms on ReachBot's chassis, (3) boom maximum extension, (4) boom cross-sectional geometry, and (5) number of active/passive degrees-of-freedom at each joint. Using first-order approximations, we analyze the relationships between these parameters and various performance metrics including stability, manipulability, and mechanical interference. We apply our method to a mission where ReachBot navigates and gathers data from a martian lava tube. The resulting design is shown in Fig. 1.

==> grasp_mat_deriv.tex <==
\subsection{Grasp stability}
\subsubsection{Attempt 1}
Consider the following ReachBot system, where $\hat{u}_i$ is the unit vector in the direction of boom $i$.
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{placeholder_figs/boom_unitvec.png}
    \caption{Boom unit vector}
    \label{fig:my_label}
\end{figure}

Consider the grasp matrix formulation from Cutkosky and Kao~\cite{cutkosky1989computing}.
\begin{equation}
    K = K_b + K_J = (^P_B J^T)\frac{\delta f_f}{\delta x_b} + \frac{\delta(^P_B J^T)f_f}{\delta x_b}
\end{equation}
Some assumptions to simplify:
\begin{itemize}
    \item $K_J = 0$ because the booms are securely attached at the shoulders and grippers (no changes in geometry due to motion)
    \item $^P_B J = I_{6x6}$ for a point mass
    \item $C_\theta = K_\theta^{-1} = I_{n x n}$ for simplification
    \item $C_s = 0$
\end{itemize}
% Because the booms are securely attached both at the shoulders and the grippers, there are no changes in geometry due to motion, so $K_J = 0$. Additionally, since $^P_B J$ represents a transformation between the object and the contact, for a point mass $^P_B J = I_{6x6}$. 
Let the joint Jacobian matrix for boom $i$ be
\begin{equation}
    J_{\theta i} = \begin{bmatrix} u_{xi} & 0 & 0 & 0 \\
                                  u_{yi} & 0 & 0 & 0 \\
                                  u_{zi} & 0 & 0 & 0 \\
                                       0 & 1 & 0 & 0 \\
                                       0 & 0 & 1 & 0 \\
                                       0 & 0 & 0 & 1 \end{bmatrix}
\end{equation}
such that
\begin{equation}
    \begin{bmatrix} \delta x \\ \delta y \\ \delta z \\ \delta\theta_x \\ \delta\theta_y \\ \delta\theta_z 
    \end{bmatrix}
    = J_{\theta i} \begin{bmatrix} \delta L \\ \delta\theta_x \\ \delta\theta_y \\ \delta\theta_z \end{bmatrix}.
\end{equation}
For this analysis, we assume that the booms can (1) extend/retract, resulting in a $\delta L$, and (2) impart an arbitrary moment on the body.
% In the simplest case, let Equation (10) in \cite{cutkosky1989computing} be
% \begin{equation}
%     C_\theta = K_\theta^{-1} = I_{n x n}.
% \end{equation}
Combining (9), (10), (14), and (15) in \cite{cutkosky1989computing}, we get
\begin{equation}
    K = K_p = C_f^{-1} = C_j = J_\theta J_\theta^T
\end{equation}

In general, $C_f$ is not invertible, so I used the pseudo-inverse. This process leads to unsatisfying results:
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{placeholder_figs/Figure_1.png}
    \caption{Minimum eigenvalue as a function of number of booms}
    \label{}
\end{figure}

\subsubsection{Attempt 2}
I also tried a Cable-driven robot approach to calculating the grasp stiffness matrix. Consider the following formulation from Behzadipour and Khajepour \cite{behzadipour2006stiffness}, given in Equation (5):
\begin{equation}
    K = J^T \Omega J + \frac{d}{dp}(J^T) \tau
\end{equation}
Again, the change in geometry is zero: $\frac{d}{dp}(J^T) = 0$. The Jacobian is derived similarly
\begin{equation}
    J_{\theta i} = \frac{dl}{dp} = \begin{bmatrix} u_{xi} & 0 & 0 & 0 \\
                                  u_{yi} & 0 & 0 & 0 \\
                                  u_{zi} & 0 & 0 & 0 \\
                                       0 & 1 & 0 & 0 \\
                                       0 & 0 & 1 & 0 \\
                                       0 & 0 & 0 & 1 \end{bmatrix}
\end{equation}
For simplicity, let $\Omega = I_{nxn}$, which means
\begin{equation}
    K = J^T J.
\end{equation}
This is the transpose of the last result, which is probably due to a misunderstanding of coordinate frames. More importantly, neither of these methods produce results that make sense to me.

==> old_missions.tex <==
\subsection{Lunar pit wall}\label{sec:moon}
The layered stratigraphy in the walls of lunar pits provides evidence to help understand the formation of the Moon's secondary crust~\cite{robinson2012confirmation}. To address questions identified by the lunar science community~\cite{NRC,Lunar exploration roadmap}, a mission to a lunar pit should scale the exposed vertical wall, taking regular measurements to gather a spatially continuous geologic record\cite{kerber2020moon}.

A representative lunar pit wall is illustrated in Fig.~\ref{fig:moon}. Lunar pit craters tend to have a funnel section that decreases the diameter of the pit from the surface to the upper wall, then after the bottleneck, the pit increases in size again via a sloping lower wall~\cite{todo}. Scientists expect these walls to have vertical layers between $5-10$m thick with shelves that protrude up to $5$m out. Additionally, the protruding shelves could have overhangs and possibly upward-facing surfaces coated in regolith dust~\cite{todo}.
Our trade study approach could find a solution here.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\columnwidth]{placeholder_figs/moon.png}
    \caption{Representative lunar pit wall.}
    \label{fig:moon}
\end{figure}

\sstodo{Payload from mission objectives -> volume, weight}\\
\sstodo{grippers (probably same as Mars)}\\
\sstodo{Workspace determination}\\
\sstodo{Performance metrics compared to Moondiver}

\subsection{Enceladus surface}\label{sec:enceladus}
The search for habitable conditions and/or evidence of life on other planets is a large focus of current space exploration. Data from Cassini indicates that the plumes of Enceladus contain organic carbon, nitrogen, and salts~\cite{mckay2014follow}, which are crucial elements of habitability. Exploring the subsurface liquid water from which these plumes originate is therefore of high importance for future missions, but likely require a mechanism for surface traversal between the landing site and the plume vent. Therefore, the focus for a surface mission to Enceladus is to carry deployable vent explorers across the icy surface.

A representative surface is illustrated in Fig.~\ref{fig:enceladus}. One of the main challenges for an Enceladus mission is that the irregularities on the surface are largely unknown, with several meters per pixel in our best resolution images. The unknown terrain geometry in conjunction with the 10-100m icy blocks that cover the surface~\cite{https://photojournal.jpl.nasa.gov/catalog/PIA06252}, highlight one of ReachBot's key advantages: the size of its footstep is not constrained by the size of the robot. This allows ReachBot to step over or navigate around obstacles several orders of magnitude larger than its body.  

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{placeholder_figs/enceladus.png}
    \caption{Representative Enceladus surface.}
    \label{fig:enceladus}
\end{figure}

\sstodo{Payload from mission objectives -> volume, weight}\\
\sstodo{grippers}\\
\sstodo{Workspace determination}\\
\sstodo{Performance metrics compared to EVE? EELS?}
